Evaluating Large Language Models on Misconceptions in Multi-Turn Medical Conversations

Patients seeking medical information often ask questions that embed incorrect assumptions or misconceptions. In such cases, safe medical communication requires not only answering the question, but identifying and correcting the underlying false belief. These interactions naturally unfold over multiple turns, a pattern now mirrored in interactions with LLMs. Yet current evaluation frameworks do not capture model behavior in these settings, where misconceptions can emerge, persist, or evolve over the course of a conversation. Whether LLMs can reliably correct such misconceptions over time remains largely unexamined. To study this, we introduce ThReadMed-QA, a multi-turn medical dialogue dataset of 2,437 patient-physician conversation threads comprising 8,204 question-answer pairs, derived from real patient interactions on AskDocs. This dataset enables systematic evaluation of whether models can detect and correct misconceptions under a multi-turn context. We evaluate five LLMs using a rubric-based LLM-as-a-Judge framework that scores responses based on their ability to identify and correct misconceptions. Our experiments reveal a consistent pattern: even frontier models that can address misconceptions in a single interaction degrade substantially over subsequent turns. GPT-5 and Claude-Haiku correct these false presuppositions around 85% on initial questions but drop to roughly 50% within two follow-ups. An oracle analysis replacing prior model outputs with physician responses shows that much of the degradation is driven by error propagation, while performance remains imperfect even under correct context. Even when models tend to correct misconceptions initially, their performance degrades substantially over later turns, leading to inconsistent and potentially unsafe guidance in patient-facing settings and highlighting the need for evaluation frameworks that capture multi-turn behavior.

==> MLHC2026-ResearchTrack-Template/latex/00_abstract.tex <==
\begin{abstract}

Patients seeking medical information often ask questions that embed incorrect assumptions or misconceptions. In such cases, safe medical communication requires not only answering the question, but identifying and correcting the underlying false belief. These interactions naturally unfold over multiple turns, a pattern now mirrored in interactions with LLMs. Yet current evaluation frameworks do not capture model behavior in these settings, where misconceptions can emerge, persist, or evolve over the course of a conversation. Whether LLMs can reliably correct such misconceptions over time remains largely unexamined. To study this, we introduce \datasetname,  a multi-turn medical dialogue dataset of 2,437 patient–physician conversation threads comprising 8,204 question–answer pairs, derived from real patient interactions on r/AskDocs. This dataset enables systematic evaluation of whether models can detect and correct misconceptions under a multi-turn context. We evaluate five state-of-the-art LLMs using a rubric-based LLM-as-a-Judge framework that scores responses based on their ability to identify and correct misconceptions. Our experiments reveal a consistent pattern: even frontier models that can address misconceptions in a single interaction degrade substantially over subsequent turns. GPT-5 and Claude-Haiku correct these false presuppositions around 85\% on initial questions but drop to approximately 50\% within two follow-ups. Additionally, GPT-4o exhibits a sharper decline, falling from 65\% to 21\%, indicating a failure to sustain safe reasoning across dialogue. An oracle analysis replacing prior model outputs with physician responses shows that much of the degradation is driven by error propagation, while performance remains imperfect even under correct context. These findings reveal a critical reliability gap in LLMs. Even when models tend to correct misconceptions initially, their performance degrades substantially over subsequent turns, leading to inconsistent and potentially unsafe guidance in patient-facing settings and highlighting the need for evaluation frameworks that capture multi-turn behavior.


\end{abstract}



==> MLHC2026-ResearchTrack-Template/latex/01_introduction.tex <==
\section{Introduction}
\label{sec:intro}

%P1 - LLM adoption and Misconceptions

LLMs are increasingly used by patients as a source of medical information, offering unprecedented accessibility to medical guidance outside traditional clinical settings \citep{costagomes2025itstimetemporalmodal}. Surveys indicate that a substantial and growing fraction of patients now seek health advice from LLMs, particularly where access to clinical care is limited \citep{kffTrackingPoll}. In these interactions, patients often ask questions that embed incorrect assumptions or misconceptions about their condition, symptoms, or treatment \citep{srikanth2024pregnant}. These misconceptions are often implicit and shaped by incomplete knowledge or prior beliefs. Safe medical communication, therefore, requires not only answering the question but also identifying and correcting the underlying false belief rather than accepting the premise as stated.


\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
\textbf{Dataset} & \textbf{User-Authored QA} & \textbf{Open-Ended} & \textbf{Multi-Turn} & \textbf{Physician-Verified} \\
\midrule
MedQA \cite{jin2020diseasedoespatienthave}             & \xmark & \xmark & \xmark & \cmark \\
PubMedQA \cite{jin2019pubmedqadatasetbiomedicalresearch}  & \xmark & \xmark & \xmark & \cmark \\
MedMCQA \cite{pal2022medmcqalargescalemultisubject}    & \xmark & \xmark & \xmark & \cmark \\
MedQA-Followup \cite{manczak2025shallow}               & \xmark & \xmark & \cmark & \cmark \\
MedRedQA \cite{nguyen2023medredqa}                     & \cmark & \cmark & \xmark & \cmark \\
MedicationQA \cite{abacha2019bridging}                 & \cmark & \cmark & \xmark & \xmark \\
HealthSearchQA \cite{53083}                            & \cmark & \cmark & \xmark & \xmark \\
\midrule
\textbf{\datasetname{} (ours)}                         & \cmark & \cmark & \cmark & \cmark \\
\bottomrule
\end{tabular}%
}
\caption{Comparison of medical QA datasets. Our dataset \datasetname \ is the first to have patient-authored questions and natural follow-ups, along with verified physician responses.} 
\label{tab:dataset_comparison}
\end{table}


%P2 - Multi-turn and the gap in evaluation 

Moreover, in clinical practice, patient–physician interactions are inherently conversational, unfolding over multiple turns as patients refine their concerns, introduce new information, or reinterpret prior guidance \citep{heritage2006communication}. This pattern is increasingly reflected in interactions with LLMs, where users engage in iterative dialogue rather than isolated queries, and misconceptions may arise at any point in the conversation (Figure~\ref{fig:example}). However, existing evaluation frameworks do not assess model behavior in these settings. Early medical QA datasets primarily emphasize factual recall and exam-style reasoning. MedQA \citep{jin2020diseasedoespatienthave}, MedMCQA \citep{pal2022medmcqalargescalemultisubject}, and PubMedQA \citep{jin2019pubmedqadatasetbiomedicalresearch} are constructed from licensing examinations or biomedical literature, offering limited insight into real-world patient interaction \citep{raji2025s, Agrawal2025TheEI}. While later datasets incorporate consumer-facing questions, including presuppositions \citep{sambara2026medredflaginvestigatingllmsredirect, zhu2025cancermythevaluatinglargelanguage}, they continue to evaluate responses in isolation \citep{abacha2019bridging, 53083, nguyen2023medredqa}. More recent efforts probe multi-turn robustness through synthetic or adversarial follow-ups, yet they do not capture how misconceptions arise and evolve in authentic multi-turn interactions that real patients have when asking medical questions around their conditions \citep{manczak2025shallow, laban2025llms}. Consequently, a critical question remains unanswered: \textbf{Can LLMs reliably identify and correct patient misconceptions as conversations unfold over multiple turns of patient-authored interactions?}

%P3 - My contributions (dataset + what it enables) 


To address this question, we introduce \datasetname, a multi-turn medical dialogue dataset derived from real patient–physician interactions on r/AskDocs. The dataset includes 2,437 conversation threads, comprising a total of 8,204 question–answer pairs.
Unlike prior resources, \datasetname \ captures how real patients iteratively seek medical guidance, preserving the natural flow of follow-up questions, clarifications, and evolving concerns across turns. As shown in Table~\ref{tab:dataset_comparison}, it is the first dataset to combine patient-authored questions, multi-turn interactions, and physician-verified responses within a single evaluation setting. This structure enables systematic evaluation of whether LLMs can identify and correct misconceptions not only at initial contact, but as they emerge, persist, or evolve throughout a conversation.

%P4 - Evaluation Framework + Tease 

We evaluate five state-of-the-art LLMs on their ability to identify and correct patient misconceptions in multi-turn conversations. Specifically, we assess whether models detect false assumptions embedded in patient questions and appropriately challenge or correct them as they arise throughout the interaction. To enable scalable evaluation, we employ a rubric-based LLM-as-a-Judge framework, validated against expert evaluations, to score how effectively models handle misconceptions. Our results reveal a consistent failure mode: models do not reliably sustain this behavior over time, with performance deteriorating as conversations unfold. This instability indicates that misconception correction by LLMs is not a persistent capability, but one that breaks down under realistic multi-turn interactions.


\subsection*{Generalizable Insights about Machine Learning in the Context of Healthcare}

Our study highlights an important gap in how patient-facing medical LLMs are currently evaluated. We show that the ability to identify and correct patient misconceptions is not a stable capability, but one that degrades as interactions progress across turns. This highlights the need to evaluate how models handle misconceptions as they emerge and evolve across interactions. By enabling evaluation on real patient-authored questions and follow-ups with physician responses, \datasetname \ provides a foundation for studying model behavior under realistic conditions. Beyond misconception handling, our proposed setup can support the evaluation of other safety-critical behaviors that emerge during interaction. Our findings suggest that future benchmarks and model development must explicitly account for interaction dynamics when evaluating patient-facing systems. To facilitate future research in this direction, we release the code \footnote{\url{https://github.com/monicamunnangi/ThReadMed-QA-Misc}} and the dataset \footnote{\url{https://huggingface.co/datasets/monicamunnangi23/threadmed-qa}}.


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{MLHC2026-ResearchTrack-Template/latex/images/example.pdf}
    \vspace{-1.5em}
    \caption{A representative conversation thread from \datasetname. Misconception can emerge early in the conversation (left) or in the later turns (right). Physicians correct these and provide safe answers irrespective of where they appear.}
    \label{fig:example}
\end{figure}

==> MLHC2026-ResearchTrack-Template/latex/02_related_work.tex <==
\section{Related Work}
\label{sec:related_work}

\paragraph{Evolution of medical QA datasets}

Early benchmarks for medical question answering primarily emphasize factual recall and exam-style reasoning. Datasets such as MedQA \citep{jin2020diseasedoespatienthave}, MedMCQA \citep{pal2022medmcqalargescalemultisubject}, and PubMedQA \citep{jin2019pubmedqadatasetbiomedicalresearch} are constructed from medical licensing examinations or biomedical literature, enabling controlled evaluation of medical knowledge but offering limited insight into real-world patient interaction \citep{raji2025s, Agrawal2025TheEI}. Subsequent efforts sought to better reflect consumer-facing use cases by incorporating health-related search queries and community-authored questions, including Medication QA \citep{abacha2019bridging}, and HealthSearchQA \citep{53083}. There are several datasets constructed from online health forums, search logs, and tele-health consultations \citep{nguyen2023medredqa, abacha2019summarization}. These datasets improve coverage of lay language and consumer concerns, yet they continue to evaluate models largely through single-turn settings. To our knowledge, \datasetname \ is the first multi-turn medical dataset with patient-authored questions and follow-ups.

\paragraph{Medical misconceptions and LLM Sycophancy}

Questions that contain misconceptions have long been studied in linguistics \citep{kaplan1978indirect, duvzi2015questions}, where the appropriate response is often to challenge or negate the incorrect presupposition. However, LLMs are known to align with users even when they are factually incorrect \citep{perez2023discovering}, termed as \textit{sycophancy}. This tendency is particularly concerning in medical contexts, where incorrect assumptions may involve diagnoses, medication safety, or symptom severity. Recent work introduced datasets to explore misconception handling in both general domain \citep{yu-etal-2023-crepe} and specific medical settings, including pregnancy and maternal health \citep{srikanth2024pregnant} and cancer care
\citep{zhu2025cancermythevaluatinglargelanguage}. However, most prior work focuses on single-turn settings \citep{sambara2026medredflaginvestigatingllmsredirect} or relies on synthetically generated questions \citep{zhu2025cancermythevaluatinglargelanguage}, which lack patient-specific context and underestimate the difficulty of real interactions where misconceptions emerge implicitly and evolve over time. Our dataset addresses this gap by enabling evaluation on authentic multi-turn patient interactions.


\paragraph{Multi-turn LLM Interaction in Medicine}

Recent work highlights a disconnect between how medical LLMs are evaluated and how they are used in practice \citep{Agrawal2025TheEI, Stanwyck2026.02.12.26346164}. Systematic reviews show that the majority of medical LLM evaluations rely on synthetic or exam-style data, with minimal use of real clinical or patient-generated text \citep{Bedi2024.04.15.24305869}. On the other hand, research reports LLMs having near-clinician accuracy in single-turn settings \citep{singhal2023towards} in some tasks, their performance degrades sharply when moving to multi-turn interactions \citep{laban2025llms}. Error propagation is also a pattern observed in  prior work on sequential and dialogue systems, showing that earlier model outputs can influence later predictions, producing compounding failures across an interaction \citep{Chen_2017, ranzato2016sequenceleveltrainingrecurrent}. In medical settings this brittleness is especially concerning: models that appear competent on static questions may fail to maintain consistency, challenge incorrect premises, or preserve appropriate safety guidance as a conversation unfolds. However, \citep{manczak2025shallow} experimented with adversarial set-ups in examination-style MCQs and does not model real patient information-seeking trajectories. Our work addresses this gap by explicitly evaluating multi-turn patient–LLM interactions grounded in authentic patient behavior.




==> MLHC2026-ResearchTrack-Template/latex/03_dataset.tex <==
\section{Dataset}

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{MLHC2026-ResearchTrack-Template/latex/images/data_pipeline.pdf}
    \caption{Dataset construction and filtering process.  We selected posts from r/AskDocs from Jan 2015 to Jun 2023, totaling approximately 1.8 million posts. After preprocessing and keeping the thread with the original poster (OP) and physician, we have the final set \textbf{comprising 8,204 question-answer pairs}, within the 2,437 conversation threads.} 
    \label{fig:filtering}
\end{figure}

We introduce \datasetname, a multi-turn medical dialogue dataset derived from real patient–physician interactions on r/AskDocs, a Reddit community where patients seek medical advice from healthcare professionals. Unlike prior QA datasets, \datasetname  \ captures extended patient–physician dialogues in which patients ask follow-up questions to clarify, refine, or challenge initial answers. 


\subsection{r/AskDocs}
We collect data from the subreddit \texttt{r/AskDocs}\footnote{\url{https://www.reddit.com/r/AskDocs/}}, an online forum where lay users seek medical advice from a community of physicians and healthcare professionals. In this setting, users post detailed descriptions of their symptoms, medical history, and concerns, and may engage in follow-up questions as the conversation evolves. Responses are often provided by community-verified medical professionals, whose credentials are reviewed by subreddit moderators and indicated through user flairs or tags (e.g., ``physician'', ``doctor''). This structure enables multi-turn, patient-physician dialogues grounded in realistic clinical communication, where initial questions are frequently refined or expanded through subsequent interaction. The forum enforces structured posting guidelines that encourage users to include relevant demographic and clinical context, leading to detailed and consistent patient queries. As a result, \texttt{r/AskDocs} provides a natural source of longitudinal patient–physician exchanges suitable for studying how misconceptions arise and are addressed by humans over the course of a conversation. 

\subsection{Dataset Construction}
Similar to prior work \cite{nguyen2023medredqa}, we collected posts from January 2015 through June 2023 from  \texttt{r/AskDocs}. We then apply standard pre-processing, following \cite{nguyen2023medredqa} to remove low-quality or incomplete content, including deleted posts and bot-generated responses. We also collected all comments from each post to reconstruct patient–physician exchanges. The same cleaning pipeline is applied to comments. An overview of the construction process is outlined in Figure~\ref{fig:filtering} and more details about pre-processing and dataset construction are in Appendix~\ref{appendix:dataset_details}.



\begin{table}[t]
\centering
\small
\begin{tabular}{p{6.5cm}rr}
\toprule
\textbf{Metric} & \textbf{Complete Dataset} & \textbf{Fully Answered Subset} \\
\midrule
\multicolumn{3}{l}{\textit{Scale}} \\
Total conversation threads & 9{,}741 & 2{,}437 \\
% Threads with at lease one medical professional response & 9{,}741 (100\%) & 2{,}437 (100\%) \\
Total number of questions & 37{,}191 & 8{,}204 \\
Total number of answered questions & 21{,}595 (58.1\%) & 8{,}204 (100\%) \\
\addlinespace[3pt]
\multicolumn{3}{l}{\textit{Conversational depth}} \\
Follow-ups per thread (min / max) & 2 / 32 & 2 / 9 \\
Follow-ups per thread (mean / median) & 2.82 / 2.0 & 2.37 / 2.0 \\
Threads with $\geq$4 turns (\%) & 3{,}792 (38.9\%) & 622 (25.5\%) \\
Threads with $\geq$5 turns (\%) & 1{,}723 (17.7\%) & 185 (7.6\%) \\
\addlinespace[3pt]
\multicolumn{3}{l}{\textit{Length (num. tokens)}} \\
Question tokens (mean) & 128.6 & 141.7 \\
Answer tokens (mean) & 74.6 & 69.5 \\
Thread tokens (mean) & 656.6 & 711.2 \\
\bottomrule
\end{tabular}
\caption{Comparison of the complete dataset and the fully answered subset. Both datasets are derived from r/AskDocs threads. The complete dataset includes all threads with three or more QA turns (9,741 threads; 37,191 questions, 58.1\% answered). The fully answered subset retains only threads where every question has a physician response (2,437 threads; 8,204 questions). Token counts use tiktoken $ cl100k\_base $.}
\label{tab:full_vs_subset}
\end{table}



\subsection{Multi-turn Construction}

We construct linear patient–physician conversation threads by retaining interactions between the original poster (OP) and verified medical professionals, identified via r/AskDocs flair. Follow-up questions are restricted to the OP to preserve coherent patient narratives. For posts with multiple comment branches, we select the branch most relevant to the original question using a word-overlap heuristic \citep{KANNAN201663}, favoring on-topic discussions. We require at least two follow-up questions per thread to ensure meaningful multi-turn structure and filter out threads with incomplete or low-quality responses.


\paragraph{Orphan Handling:} Some threads contain unanswered follow-up questions, which we refer to as \textit{orphans}. To enable evaluation with complete ground-truth responses, we construct a fully answered subset by retaining only threads in which every question has a physician response. After filtering, we obtain our primary dataset of 2,437 conversation threads comprising 8,204 question–answer pairs.


Table~\ref{tab:full_vs_subset} summarizes key statistics of the dataset. The complete collection contains 9,741 conversation threads (37,191 question–answer pairs), while the fully answered subset used for evaluation contains 2,437 threads (8,204 pairs). The data span 2015-2023, covering a period of increasing reliance on online medical advice. Conversations often involve patients providing detailed context (mean of 129 tokens) and refining their concerns through follow-up questions, while physician responses tend to be more concise (mean of 75 tokens) and targeted. This asymmetry reflects realistic patient–physician communication and creates a setting where misconceptions by patients may be introduced, clarified, or persist across turns.


==> MLHC2026-ResearchTrack-Template/latex/04_methods.tex <==
\section{Methods}
\label{sec:method}

\subsection{Misconception Identification}

We first identify questions that contain medical misconceptions. Each question is labeled using an LLM-based classifier as containing a misconception if it embeds an incorrect assumption or false presupposition about a medical condition, treatment, or outcome. LLM-as-a-Judge was validated on a subset of 310 questions against physician judgment with an agreement rate of 90\% and Cohen’s $\kappa$ = 0.72 (\textit{substantial agreement}, following \cite{zhu2025cancermythevaluatinglargelanguage, pmlr-v298-munnangi25a} in the clinical domain). We provide detailed information on validation in Appendix~\ref{apx:llm-judge-validation}.  We retain all conversation threads containing at least one such question, yielding a subset of 505 conversation threads used for evaluation. We provide the full prompt in the Appendix~\ref{apx:prompts}.

\subsection{Multi-Turn Inference}

For each thread, models generate responses sequentially with full conversational context. At turn $t$, the model receives all prior patient questions and its own previous responses:

\begin{quote}
\small
\texttt{[User]:} $\langle q_0 \rangle$ \\
\texttt{[Assistant]:} $\langle a_0 \rangle$ \\
\texttt{[User]:} $\langle q_1 \rangle$ \\
\texttt{[Assistant]:} $\langle a_1 \rangle$ \\
\texttt{[User]:} $\langle q_2 \rangle$ \\
\quad $\vdots$
\end{quote}

Each response conditions on all prior model outputs, such that the model's own previous answers form part of the context for subsequent turns.

\subsection{Models}

We evaluate five state-of-the-art LLMs spanning the proprietary frontier and open-source categories:
GPT-5~\citep{OpenAI_2025} (snapshot: \texttt{gpt-5-2025-08-07}),
GPT-4o~\citep{openai2024gpt4ocard},
Claude Haiku 4.5~\citep{Claude-haiku} (snapshot: \texttt{claude-haiku-4-5-20251001}),
Gemini 2.5 Flash~\citep{comanici2025gemini25pushingfrontier},
and Llama~3.3--70B-Instruct~\citep{grattafiori2024llama}.
All models are evaluated zero-shot with no specific system prompt,  no few-shot examples, or medical-domain specialization are applied, assessing out-of-the-box capability. Temperature is set to 0 for all models that support it. We only experiment with general-domain state-of-the-art models, as numerous studies, including \cite{jeong-etal-2024-medical} and \cite{ceballos-arroyo-etal-2024-open}, have shown that domain-specific models often underperform and are rarely deployed in patient-facing interfaces. 


\subsection{Evaluation Framework}

We evaluate model responses using a rubric-based LLM-as-a-judge framework, following \citet{zhu2025cancermythevaluatinglargelanguage}. Each response is scored on a three-point scale (full prompt in Appendix~\ref{apx:prompts}):

\begin{itemize}
    \item \textbf{Score -1:} The answer fails to recognize or acknowledge false presuppositions in the
    questions
    \item \textbf{Score 0:} The answer appears aware of false presuppositions but often struggles to identify them clearly, or does not fully address them with the correct information
    \item \textbf{Score 1:} The answer accurately addresses the false presuppositions, providing comprehensive responses that clarify misunderstandings or question the presuppositions
    
\end{itemize}

% The judge is validated against physician responses on a held-out subset to ensure alignment with clinical reasoning.
We validate our LLM-as-a-Judge with physician judgment, with an agreement rate of 87.14\% and Cohen's $\kappa$ = 0.68 (\textit{substantial agreement}). We provide detailed information on validation in Appendix~\ref{apx:llm-judge-validation}. We also adapt multiple models as LLM judges and aggregate the scores to de-bias the judgments (more information in Appendix~\ref{apx:llm-judge-validation}) following prior work \cite{wataoka2025selfpreferencebiasllmasajudge}. 

\subsection{Metrics}

\subsubsection{Single-turn Metrics:} We adopt single-turn metrics from \citet{zhu2025cancermythevaluatinglargelanguage}. PCR (Presupposition Correction Rate) measures the proportion of responses that correctly address the misconception (score $=1$), while PCS (Presupposition Correction Score) is the average score over $\{-1, 0, 1\}$, capturing partial and incorrect responses.

\subsubsection{Multi-turn Metrics:}

To analyze model behavior over the course of a conversation, we extend single-turn metrics to the multi-turn setting.

\paragraph{Per-turn Performance:}
We compute the Presupposition Correction Rate (PCR) at each turn $t$:
\begin{equation}
    \text{PCR}_t = \frac{1}{N_t} \sum_{i=1}^{N_t} \mathbb{I}[s_{i,t} = 1]
\end{equation}
where $s_{i,t} \in \{-1, 0, 1\}$ is the score for example $i$ at turn $t$, and $N_t$ is the number of evaluated instances at that turn and $\mathbb{I}(\cdot)$ is the indicator function, equal to 1 if the condition holds and 0 otherwise.


\paragraph{Recovery Rate:}
We measure the ability of models to recover from prior failures in misconception correction across turns. Specifically, we compute the conditional probability that a model correctly resolves a misconception at turn $t+1$ given that it failed to do so at turn $t$:
\begin{equation}
    \text{RR} = P(s_{t+1} = 1 \mid s_t \neq 1)
\end{equation}
where $s_t \in \{-1, 0, 1\}$ denotes the score at turn $t$. Higher values indicate that a model is more likely to recover and correctly address a misconception after previously failing. We estimate this probability over all consecutive turn pairs $(t, t+1)$ where both turns are labeled as containing misconceptions.

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{MLHC2026-ResearchTrack-Template/latex/images/baseline_vs_oracle.pdf}
    \caption{Example of multi-turn misconception handling under two inference settings. The same patient-authored conversation is shown with different model responses. On the left, the model generates responses conditioned on its own previous outputs, leading to failure to explicitly address the misconception (“\textit{I most definitely have a concussion}”) and resulting in incomplete guidance (score: 0). On the right, (\textit{oracle -physician})the model produces a response that correctly identifies and challenges the underlying false presupposition while providing appropriate medical advice (score: 1).}
    \label{fig:baseline_vs_oracle}
\end{figure}


\subsection{Oracle Physician Ablation}

To separate the effect of question difficulty and embedded false presuppositions from errors introduced by prior model-generated context, we conduct an oracle-style ablation in which all preceding turns use verified physician responses from the r/AskDocs thread, rather than the model’s own prior outputs.


For each multi-turn thread, let patient turns be indexed as $t = 0, 1, \ldots, T-1$. For each target turn $t \geq 1$, we construct the input by concatenating the dialogue history up to that turn. Specifically, for each $i < t$, we include the patient question $Q_i$ and the corresponding physician response $A^{\mathrm{phys}}_i$. For the target turn, we append only the patient question $Q_t$, which the model must answer. Under this setup, the model conditions exclusively on the oracle (physician) context and never on its own prior generations. Since turn $t = 0$ has no preceding in-thread physician responses, oracle prompts are defined only for $t \geq 1$. We report PCR (\%) and Uncorrected (\%) in this setting to assess the impact of oracle context on model behavior. We illustrate this setup in Figure~\ref{fig:baseline_vs_oracle}.





==> MLHC2026-ResearchTrack-Template/latex/05_results.tex <==
\section{Results}

\begin{figure}[t]
\centering
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{MLHC2026-ResearchTrack-Template/latex/images/pcr_plot.pdf}
    \centerline{\hspace*{2.2em}\small (a)}
\end{minipage}
\hfill
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{MLHC2026-ResearchTrack-Template/latex/images/uncorrected.pdf}
    \centerline{\hspace*{2.2em}\small (b)}
\end{minipage}
\caption{Overall misconception correction performance across models. (a) PCR (\%) shows correction rates \textbf{aggregated across all turns}. (b) Uncorrected response rates (\%), including both partially correct (0) and incorrect ($-1$) responses, \textbf{aggregated across all turns}, indicate how often models fail to fully resolve misconceptions.}
\label{fig:mean_results}
\end{figure}

Figure~\ref{fig:mean_results} summarizes overall misconception correction \textbf{performance aggregated across all turns}. As shown in Figure~\ref{fig:mean_results}(a), frontier models achieve higher correction rates, with Claude Haiku and GPT-5 exceeding 60\% PCR, while Gemini 2.5 Flash performs moderately (43.0\%). In contrast, GPT-4o and Llama 3.3--70B show substantially lower correction rates. Figure~\ref{fig:mean_results}(b) provides a complementary view by reporting the proportion of responses that fail to fully correct misconceptions. These uncorrected rates remain high across all models, exceeding 35\% even for the strongest systems and rising above 65\% for weaker models. This indicates that even when evaluated across all turns, models frequently provide incomplete or incorrect responses to misconception-laden questions.

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{MLHC2026-ResearchTrack-Template/latex/images/turn_by_turn_pcr_mean_with_ci.pdf}
    \caption{Multi-turn Presupposition Correction Rate (PCR) across models with confidence intervals (CI). Performance consistently degrades as conversations progress, with all models exhibiting substantial drops after the initial turn. Even frontier models such as Claude Haiku and GPT-5 show marked declines, while weaker models degrade further and remain at low performance across turns.}
    \label{fig:pcr_turn_by_turn}
\end{figure}


\subsection{Observed Correction Rates Decline at Later Turns}

We next analyze model performance across turns within a conversation by measuring PCR at each turn. As shown in Figure~\ref{fig:pcr_turn_by_turn}, performance decreases consistently as conversations progress. Even frontier models that achieve strong initial performance fail to sustain this behavior over time. GPT-5 starts at 88.1\% PCR at the first turn but drops to 48.0\% by turn 2, a reduction of over 40 percentage points. Similarly, Claude Haiku declines from 84.4\% to 53.5\% over the same span, indicating that initial success does not translate into stable multi-turn performance. This effect is more pronounced for weaker models. GPT-4o drops from 65.1\% at the first turn to 21.2\% by turn 2, while Llama 3.3--70B falls from 55.0\% to 17.7\%. At these levels, most misconception-laden queries are no longer correctly addressed. We report detailed results in Appendix~\ref{apx:add_results}.

Across all models, the largest drop occurs within the first few turns, after which performance stabilizes at substantially lower levels. Overall, these results show that misconception correction is not a stable capability, and models struggle to maintain it as conversations unfold.

\begin{table}[h!]
\centering
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{lccc}
\toprule
\textbf{Model} & \textbf{RR (\%)} & \textbf{95\% CI} & \textbf{\# Failure-Start Pairs} \\
\midrule
Claude Haiku      & 51.9 & (33.3, 69.6) & 27 \\
GPT-5             & 25.9 & (9.5, 45.0) & 27 \\
Gemini 2.5 Flash  & 21.7 & (10.4, 35.3) & 46 \\
GPT-4o            & 12.8 & (4.3, 23.4) & 47 \\
Llama 3.3--70B    & 13.8 & (5.7, 23.6)  & 65 \\
\bottomrule
\end{tabular}
\caption{Recovery rate (RR) across models with 95\% bootstrap confidence intervals (1000 bootstrap iterations). RR measures the probability that a model correctly resolves a misconception at turn $t+1$ given failure at turn $t$. \# Failure-Start Pairs denotes the number of consecutive turn pairs where the model failed at turn $t$.}
\label{tab:recovery_rate}
\end{table}


\subsection{Limited Recovery Across Turns}

While the previous analysis shows that performance declines across turns, we next examine whether models can recover after an initial failure. Table~\ref{tab:recovery_rate} reports recovery rates (RR) with 95\% confidence intervals estimated via bootstrap resampling (1{,}000 iterations). Because RR is conditioned on prior failure, the evaluated instances differ across models; consequently, RR should not be interpreted as a strict ranking of model capability, but rather as a diagnostic measure of how difficult it is for models to recover once an incorrect conversational trajectory has been established.

Recovery remains limited across all systems, indicating that once a model fails to correct a misconception, it is unlikely to recover in subsequent turns. Even stronger models show only partial recovery. Claude Haiku achieves the highest recovery rate at 51.9\% (33.3--69.6), while GPT-5 recovers in only 25.9\% (9.5--45) of cases following a failure. Recovery is substantially lower for weaker models, with GPT-4o and Llama 3.3--70B below 15\%, and confidence intervals reflecting high uncertainty due to the limited number of failure-start pairs.

Taken together, these results suggest that once models fail to identify or correct a misconception, recovery is uncommon. Although RR is conditioned on model-specific failures and is not intended for direct cross-model comparison, it highlights a shared vulnerability where models struggle to recover from erroneous conversational trajectories.


\begin{figure}[t]
\centering
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{MLHC2026-ResearchTrack-Template/latex/images/oracle_pcr_plot.pdf}
    \vspace{-2mm} % Adjust this to move (a) up or down
    \centerline{\hspace*{2.2em}\small (a)}
\end{minipage}
\hfill
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{MLHC2026-ResearchTrack-Template/latex/images/oracle_uncorrected.pdf}
    \vspace{-2mm} % Adjust this to move (a) up or down
    \centerline{\hspace*{2.2em}\small (b)}
\end{minipage}

\caption{Oracle evaluation using physician-provided context. (a) PCR (\%) aggregated over all turns and (b) uncorrected response rates (\%), aggregated over all turns, when prior turns are replaced with gold physician answers. Improvements relative to the standard setting indicate the impact of error propagation from model-generated context.}
\label{fig:mean_oracle_results}
\end{figure}

\subsection{Oracle Physician Context Substantially Improves Performance}

To isolate the effect of conversational context, we evaluate models in an oracle setting where prior turns (LLMs' responses) are replaced with physician-provided responses. This removes error accumulation from earlier model outputs and allows us to assess performance when conditioned on the correct context. Figure~\ref{fig:mean_oracle_results} shows that all models improve substantially under the oracle context. Correction rates increase across the board, indicating that a significant portion of multi-turn degradation arises from error propagation. For example, GPT-5 achieves 87.4\% PCR, up from 62.4\%, while Claude Haiku reaches 75.8\% PCR, up from 60.6\%. Even weaker models show notable gains, with GPT-4o and Llama 3.3--70B approaching 50\% PCR under oracle context.

Overall, models continue to exhibit high rates of uncorrected responses, particularly for weaker systems, suggesting that correct context alone is insufficient to fully resolve misconception handling. Additionally, these results indicate that error propagation is a major contributor to multi-turn degradation, but intrinsic limitations in identifying and correcting misconceptions remain an important source of failure.

\paragraph{Turn Difficulty \& Oracle Style Shifts:} To fully isolate error propagation from both question difficulty and style shifts, we perform another ablation "target-turn", and summarize the results in the following table~\ref{tab:conversation_settings}. This setting provides the patient’s prior questions but removes all prior responses (model or physician). Results show that removing prior model responses significantly improves performance (e.g., GPT-5 improves from 60.6\% to 76.3\%), confirming that models actively propagate their own errors, though a gap below the Oracle remains due to intrinsic difficulty.

\begin{table}[t]
\centering
\begin{tabular}{lccc}
\toprule
\textbf{Model} & \textbf{Multi-turn} & \textbf{Target-Turn} & \textbf{Oracle} \\
\midrule
GPT-5          & 60.6 & 76.3 & 87.4 \\
Claude Haiku   & 62.4 & 60.3 & 75.8 \\
Gemini Flash   & 43.0 & 34.1 & 59.8 \\
GPT-4o         & 34.3 & 37.7 & 59.1 \\
Llama 3.3 70B  & 26.5 & 26.7 & 49.3 \\
\bottomrule
\end{tabular}
\caption{Presupposition Correction Rate (PCR, \%) across conversational settings. Multi-turn uses model-generated conversation history, Target-Turn evaluates questions independently without prior context (responses), and Oracle conditions on physician responses. Higher Oracle performance suggests that error propagation from previous model responses is a major contributor to multi-turn degradation.}
\label{tab:conversation_settings}
\end{table}

==> MLHC2026-ResearchTrack-Template/latex/06_discussion.tex <==
\section{Discussion}
\label{sec:discussion}

Patients often ask questions built on incorrect assumptions, requiring AI systems not just to answer but to identify and correct the underlying misconception \citep{srikanth2024pregnant}. These misconceptions can evolve across multi-turn conversations, as patients reinterpret prior guidance from the AI system. Yet existing evaluation frameworks mostly test isolated questions, missing how misconceptions emerge, persist, and shift over the course of a dialogue \citep{Agrawal2025TheEI, Bedi2024.04.15.24305869}.

Our results show that strong single-turn performance does not guarantee reliability over the course of a conversation. While several models demonstrate strong correction ability at the initial turn, this ability degrades rapidly as conversations progress, with substantial declines within the first few follow-ups. As performance drops, misconceptions increasingly go unresolved, and errors tend to persist rather than being corrected in later responses. This pattern suggests that turns are not independent: a missed correction shapes the context for everything that follows, producing path-dependent failures rather than isolated ones. This is consistent with prior work on sequential and dialogue systems \citep{bigham2017deaf}, where earlier outputs influence later predictions and compound into larger failures over an interaction \citep{Chen_2017, ranzato2016sequenceleveltrainingrecurrent}.

The oracle-physician ablation supports this interpretation: replacing prior model-generated responses with physician answers consistently improves performance across all models, indicating that some of the decline is driven by earlier model outputs rather than the difficulty of any single turn. However, performance still falls short of perfect for some models even with this oracle context, suggesting that clean prior context alone is not sufficient. Together, these results point to two distinct contributors to failure: propagation of earlier errors, and the underlying difficulty of catching misconceptions at all.

These findings carry implications for how LLMs are evaluated and deployed in patient-facing settings. Benchmarks based on isolated queries miss the temporal dynamics observed here and can overestimate reliability in real interactions. Multi-turn evaluation reveals failure modes hidden in single-turn settings, including performance decline, persistence of errors, and limited recovery after mistakes \citep{laban2025llms, manczak2025shallow, dongre2025drift}. Evaluation should account for interaction dynamics, not just single-turn accuracy.

This also points to a design implication. Since much of the decline traces back to uncorrected errors compounding over time, brief points of human input could break that chain \citep{morris2017subcontracting}. One approach is lightweight micro-interactions, where a physician or other healthcare worker flags a response mid-conversation or can manually provide a correction \citep{savage2016botivist}, giving the model a chance to correct course before the error shapes later turns. The oracle-physician ablation supports the potential value of this: even partial, intermittent physician input could meaningfully improve responses over time.

More broadly, this also suggests a role for multi-stakeholder system design \citep{savage2022global}, where different healthcare workers contribute different kinds of oversight: physicians catching clinical errors, while nurses or care navigators watch for communication breakdowns or signs that a patient has misunderstood guidance. Distributing oversight this way could be more scalable than relying on physicians alone, since not every error requires the same level of expertise to catch, and it better reflects how care is delivered across multiple roles.

Beyond misconception handling, \datasetname\ offers a realistic testbed for studying broader phenomena in longitudinal interactions, including error accumulation, safety drift, and sensitivity to evolving user input. Future work could use the dataset to develop and evaluate models built for multi-turn reliability. For instance, approaches that explicitly incorporate feedback, correction, and consistency across turns, or to fine-tune and align models to better detect and resolve misconceptions in realistic patient interactions. This matters most in clinical contexts, where uncorrected early errors can compound into larger misinformation over the course of an interaction.

==> MLHC2026-ResearchTrack-Template/latex/07_limitations.tex <==
\paragraph{Limitations}

Several limitations of this work warrant consideration. First, the ground truth responses are drawn from r/AskDocs, an online forum, and are not equivalent to formal clinical documentation. Although responses are provided by verified physicians and subject to moderation, they may vary in completeness and reflect differences in clinical judgment, introducing potential noise in the reference answers. We only use the responses for oracle-physician ablation in this work. Second, the dataset is derived from Reddit and may reflect platform-specific biases. The user population is not representative of the general patient population, and interactions often follow informal, iterative patterns shaped by the platform. In addition, our filtering procedure retains only multi-turn threads with follow-up questions and a fully answered subset, which may over-represent more complex or engaged interactions and under-represent simpler, single-turn queries. Third, misconception identification and response evaluation rely on an LLM-as-a-Judge framework. Despite strong agreement with physician annotations, this approach may introduce labeling noise that can affect downstream metrics. Fourth, the number of failure-start pairs used to estimate recovery rates is limited, resulting in wide confidence intervals and restricting the strength of conclusions regarding recovery behavior. Fifth, comparisons between GPT-5 and other models should be interpreted cautiously, as GPT-5 outputs are stochastic while other models are evaluated deterministically. Finally, the dataset is restricted to English-language text and does not include multi-modal inputs, which are common in real clinical settings. 

\paragraph{Ethical Considerations}
While Reddit posts are publicly available, we recognize that users may not have originally intended their queries for large-scale research. To prioritize privacy, we strictly adhered to Reddit’s API terms of use and performed rigorous de-identification. We removed all usernames, post IDs, and specific timestamps, replacing them with unique anonymized identifiers (e.g., THREAD\_001). No metadata that could lead to the re-identification of specific Reddit threads or users was included in our analysis. 
